Point Cloud Compression with Implicit Neural Representations: A Unified Framework

Point clouds have become increasingly vital across various applications thanks to their ability to realistically depict 3D objects and scenes. Nevertheless, effectively compressing unstructured, high-precision point cloud data remains a significant challenge. In this paper, we present a pioneering point cloud compression framework capable of handling both geometry and attribute components. Unlike traditional approaches and existing learning-based methods, our framework utilizes two coordinate-based neural networks to implicitly represent a voxelized point cloud. The first network generates the occupancy status of a voxel, while the second network determines the attributes of an occupied voxel. To tackle an immense number of voxels within the volumetric space, we partition the space into smaller cubes and focus solely on voxels within non-empty cubes. By feeding the coordinates of these voxels into the respective networks, we reconstruct the geometry and attribute components of the original point cloud. The neural network parameters are further quantized and compressed. Experimental results underscore the superior performance of our proposed method compared to the octree-based approach employed in the latest G-PCC standards. Moreover, our method exhibits high universality when contrasted with existing learning-based techniques.

==> RW.tex <==
\subsection{Point Cloud Compression}

The PCC standardization encompasses two distinct compression approaches: video-based PCC (V-PCC) and geometry-based PCC (G-PCC). V-PCC projects a 3D object to multiple 2D planes and then utilizes existing image and video codecs. In contrast, G-PCC represents the voxelized point cloud geometry with an octree. The occupancies of all nodes form a binary string and can be compressed by entropy coding. G-PCC also provides another geometry coding technique, known as trisoup, which approximates the object surface using triangle meshes. For attribute compression, G-PCC uses linear transforms based on the geometry, one of which is the region-adaptive hierarchical transform (RAHT) \cite{de2016raht}. In addition, G-PCC has further improved its performance with better entropy coding and prediction of RAHT coefficients.

Recently, learning-based point cloud compression approaches has shown superior rate-distortion performance. Most of these works are based on the autoencoder architecture, where an encoder network transforms the input point cloud into latent representation and a decoder network reconstructs the input. Among these works, \cite{wang2021learnedpcgc, guarda2020adlpcc, wang2021pcgcv2, liu2022pcgformer, wang2022sparsepcgc} use 3D dense or sparse convolutional autoencoders to represent the occupancies of voxelized point cloud geometry. \cite{wang2022sparsepcac, zhang2023scalablepcac} also utilize 3D sparse convolutions in point cloud attribute compression. In contrast to these voxel-based approaches, \cite{huang20193dpcgc, sheng2021deeppcac} use PointNet-style architectures and directly compress raw points instead of voxel grids. All these learning-based approaches require training datasets (e.g., ShapeNet \cite{chang2015shapenet}) for their autoencoders. However, as discussed in \cite{alexiou2020unified}, the selection of training data can significantly affect the network's performance on testing data, which brings forward higher requirement on the generalization of the network.

\subsection{Neural Implicit Representation}

In recent years, deep neural networks are used to represent continuous 3D shapes implicitly. Such networks learn continuous volumetric functions that take 3D coordinates as input and output the corresponding features, such as signed distance function \cite{park2019deepsdf, jiang2020ligr}, occupancy function \cite{mescheder2019occnet, peng2020convoccnet} and inside/outside function \cite{chen2019imnet, genova2020ldif}. Some of these works assign latent vectors to different shapes, and condition these latent vectors on the same network, enabling a single network to represent multiple 3D shapes. The latent vectors can be either regressed by an encoder \cite{jiang2020ligr, mescheder2019occnet, chen2019imnet} or jointly optimized along with the decoder in the autodecoder architecture \cite{park2019deepsdf}.

Besides 3D shape reconstruction, coordinate-based neural networks have been applied in other areas, e.g., view synthesis, 3D interpolation, and point cloud compression. The authors in \cite{mildenhall2021nerf} proposes the neural radiance field (NeRF), which maps the 5D coordinate (spatial location and viewing direction) to the volume density and view-dependent emitted radiance. NeuralPCI \cite{zheng2023neuralpci} defines the spatial-temporal neural field that maps the 4D coordinate to the motions. The most relevant works to ours are given by \cite{hu2022nvfpcc} and \cite{isik2022lvac}, which utilize neural implicit representations to compress point cloud geometry or attribute. \cite{hu2022nvfpcc} trains a convolutional neural network along with input latent codes, where the network uses each latent code to reconstruct a group of points. \cite{isik2022lvac} represents the attributes of each point using a coordinate-based network, along with latent vectors as local parameters. In our work, we use two networks to represent point cloud geometry and attribute, respectively. Unlike these two works, we directly represent the spatial locations with global coordinates and not use any local latent vectors.
